Error-Aware Policy Learning: Zero-Shot Generalization in Partially Observable Dynamic Environments

Simulation provides a safe and efficient way to generate useful data for learning complex robotic tasks. However, matching simulation and real-world dynamics can be quite challenging, especially for systems that have a large number of unobserved or unmeasurable parameters, which may lie in the robot dynamics itself or in the environment with which the robot interacts. We introduce a novel approach to tackle such a sim-to-real problem by developing policies capable of adapting to new environments, in a zero-shot manner. Key to our approach is an error-aware policy (EAP) that is explicitly made aware of the effect of unobservable factors during training. An EAP takes as input the predicted future state error in the target environment, which is provided by an error-prediction function, simultaneously trained with the EAP. We validate our approach on an assistive walking device trained to help the human user recover from external pushes. We show that a trained EAP for a hip-torque assistive device can be transferred to different human agents with unseen biomechanical characteristics. In addition, we show that our method can be applied to other standard RL control tasks.

==> OLDINTRO.tex <==
Assistive robots that provide physical assistance have the potential to enable or augment the capability of individuals with motor impairments to complete day-to-day tasks and maintain independence. An immediate concern in developing such an autonomous and powered robot is the safety of human users because exhaustively testing the control policies on human subjects is infeasible and risky. Alternatively, one can develop policies that physically interact with humans in a simulated environment before deploying them on real users. Since safety of the user is not a concern in simulation, we can employ a number of approaches to train the control policy, without being limited by sample efficiency or computation time of the methods. 

Sidestepping from the challenge of synthesizing humans with variations, collecting human data that cover a wide range of observable variations is a relatively feasible task routinely performed by researchers in Biomechanics and Compute Animation. For example, numerous datasets of locomotion recorded from people with various biometrics are publicly available . Utilizing these human datasets, one could potentially build multiple human dynamic models varied by the observable parameters (e.g. the height) and train a universal policy conditioned on the observable parameters. This approach might generalize well when all model parameters are observable to the policy, which is unfortunately not the case of human dynamics. When the dynamic system is largely unobservable, the generalizability of the universal policy reduces to a robust policy typically trained by domain randomization techniques. Since a robust policy treats variations in the environment as noise, it has difficulty generalizing to environments with high variance, which is unfortunately the case with  human dynamics.

==> OldText.tex <==
%METHOD SECTION TEXT

%Environments with high variance pose significant challenges to robust policies trained by domain randomization approaches, while highly unobservable dynamic models often make an universal policy ineffective, because a universal policy essentially reduces to a robust policy when most parameters are unobservable.


%Our key hypothesis is that a policy can self-correct its own behavior if it is explicitly aware of the differences between what is expected in simulation and what is executed in reality. We propose a novel \emph{Error-Aware Policy} (EAP), which takes as input the reality gap represented as the deviation in the future states, referred to as "the error", and adjusts its action on-the-fly accordingly.


% Predicting error is hard. Why?
%However, predicting errors is not a straightforward problem. If we can observe all the model parameters in the target environment, we can obtain the optimal trajectory in a simulated environment and leverage it to compute the error at testing. This approach is not applicable if we cannot accurately identify the system dynamics due to many unobservable model parameters. Also, we cannot simply use a nominal trajectory for all the scenarios because the target dynamics have high variance. Therefore, we need a structured method to generate various errors in simulation and to train a robust error-aware policy.

% Introduce Universal Dynamics Model and Error Prediction Function.
%Our method utilizes a highly versatile dynamics model, \emph{Universal Dynamics Model} (UDM), which is parameterized by \emph{observable model parameters}, $\boldsymbol{\mu}_o$. The UDM allows us to configure various reality gaps by setting different model parameters and data sets. Then we can learn an error prediction function, $e: (\mathbf{s}, \mathbf{a}, \boldsymbol{\mu}_o) \mapsto \mathbb{R}^n$ that predicts the deviation of the next state between the source and the target environments, conditioned on the same state, the same action, and the same observable model parameters. The output of $e$ is passed into our error-aware policy for computing the optimal action.

% Our method utilizes the data from the target environment to train a "Universal Dynamic Model" parameterized by the \emph{observable model parameters}, $\boldsymbol{\mu}_o$. Consequently, various reality gaps can be created by using different $\boldsymbol{\mu}_o$ to train separate dynamic models to represent the source and target environments. By conditioning on $\boldsymbol{\mu}_o$, the universal dynamic models can predict the next state more accurately and provide a physical interpretation for the reality gaps.

% To utilize the engineered reality gaps during training, we propose to learn a function that characterizes the effect of a reality gap. Specifically, we learn an error function, $e: (\mathbf{s}, \mathbf{a}, \boldsymbol{\mu}_o) \mapsto \mathbb{R}$ that predicts the deviation of the next state between the source and the target environments, conditioned on the same state, the same action and the same observable model parameters. The output of $e$ is passed into the policy for computing the optimal action. We call our policy "error-aware policy".

% Combining the learned "universal dynamic models" and the "error-aware policy", our method fully utilizes all the available data from the target environment and measurable model parameters to prepare the policy for sim-to-real transfer. Our method assumes that the reality gap is caused by over-fitting the dynamic model to a small amount of data from the target environment. However, reality gaps can be caused by other factors such as, erroneous or noisy sensors or actuators, which are not addressed by this work.


%\subsection{Observable and Unobservable Parameters}
% Observable/unobservable parameters
%A dynamic system can be characterized by a set of parameters, $\bm{\mu}$. Unlike simulated environments, the parameters for real-world systems can be split into two groups $\bm{\mu} = [\bm{\mu}_o; \bm{\mu}_u]$: observable $\bm{\mu_{o}}$ and unobservable parameters $\bm{\mu_{u}}$. Typical examples of observable parameters $\bm{\mu_{o}}$ include masses, inertia matrices, or link lengths, which can be measured by conducting simple experiments. Some other dynamics, such as joint slackness, actuator dynamics, or sensor noise, are straightforward to find proper explicit parameterization or identify accurate parameters. 

% Human examples
%One extremely complex and yet important dynamic system is the human musculoskeletal system. One can often measure the height, the weight and other geometric properties of the body of a person, but complete system identification requires us to identify all the detailed parameters for many subsystems, such as bones, muscles, and neural systems, which are typically hard to measure. This motivates our algorithm to overcome the sim-to-real gap even with many unobserved dynamics parameters.

% A complex dynamic system in the real world often can only be partially characterized by a set of observable parameters, $\bm{\mu}_o$, while many other parameters that affect the dynamics of the system are unknown or immeasurable. One extremely complex and yet important dynamic system is the human musculoskeletal system. One can often measure the height, the weight and other geometry properties of the body of a person, but hundreds of other parameters are typically unknown. Similarly, some of the parameters in a complex robotic system, such as inertial and geometry properties can be easily measured, but other quantities, such as joint friction and damping are difficult to estimate. We define those un-observable parameters as $\bm{\mu}_u$ and together the dynamic parameters can be represented as a vector $\bm{\mu} = [\bm{\mu}_o, \bm{\mu}_u]$.

% % Parameters in robotics
% Typically, the dynamics of a robotic system is determined by parameters such as mass, inertia, center of mass (COM) positions, joint damping, friction, etc.. Some of these parameters are easily measurable, for example, mass and rigid-body link lengths we call these quantities observable $\bm{\mu_{o}}$. Whereas some quantities are difficult to estimate, like joint damping and friction, etc..  we call these quantities un-observable $\bm{\mu_{u}}$. Together, these parameters can be represented as a vector $\mu = [\mu_o,\mu_u]$. 

\begin{comment}
\subsection{Universal Dynamic Model (UDM)} \label{sec:universal}
% \textcolor{blue}{ Karen's notes : 
% 1)Distinction between observable and unobservable model parameters in dynamic models.
% 2)Define universal dynamic models.
% 3)Talk about how we collect data. First, human data from the real world. What are the observable parameters? 4)Second, if we don't have real world data, we can vary model parameters in a simulator and generate data for training the dynamic models.
% 5)Talk about training and loss function.
% 6)Talk about how we partition data to create reality gap}

We assume that a dynamic system can be characterized by a set of observable parameters $\bm{\mu}_o$ along with other unknown and unobservable factors. Take human musculoskeletal system as an example. We can often measure the height, the weight and other geometric properties of the body of a person, but other factors that influence the dynamics of the system are opaque to us. Against this backdrop, the first step of our approach is to learn a Universal Dynamics Models (UDM) from data collected in the target environment. A UDM $P_{\vc{\theta}}(\vc{s}'|\vc{s},\vc{a},\bm{\mu}_o)$, parameterized by $\vc{\theta}$, takes as input the current state $\vc{s}$, the action $\vc{a}$, and the observable model parameters $\bm{\mu}_o$ and predicts the next state $\vc{s}'$. 
We learn a UDM using a Long Short Term Memory (LSTM) architecture with a history of ten previous states by minimizing the following loss function:
\begin{equation} \label{eq:universal_dynamics}
    L(\bm{\theta}) =  \sum_{(\vc{s},\vc{a}, \bm{\mu}_{o}, \vc{s}') \in D} \log p_{\theta}(\vc{s}'|\vc{s},\vc{a},\bm{\mu}_{o}),
%    L(\bm{\theta}) = \sum_{i = 1}^{n} \sum_{(\bm{s}_{t},\bm{a}_{t}, \bm{\mu}_{o_i}, \bm{s}_{t+1}) \in D_{\mu_{o_i}}} \log p_{\theta}(\bm{s_{t+1}}|\bm{s_t},\bm{a_t},\bm{\mu_{o_i}})
\end{equation}
where $D = \{(\vc{s},\vc{a},\bm{\mu}_o, \vc{s}')\cdots\}$ is the pre-collected data set.

\noindent\textbf{Data collection.}
We collect the training data for UDM using two different processes for different experiments. For human experiments, we use a public dataset, such as over-ground human walking reported in the work of Fukuchi et al. \cite{dataset2018}. The dataset includes steady-state walking data for $40$ different healthy adults with ages ranging from $21$ - $87$. To compute the joint torque trajectories from the kinematic human data, we solve an inverse dynamic problem by training a policy to track the kinematic human data~\cite{peng2018deepmimic,kumar2019learning}. For other experiments on simulated agents, we create a set of agents with varying model parameters $\bm{\mu} = (\bm{\mu}_o, \bm{\mu}_u)$, which comprise observable parameters $\bm{\mu}_o$ and unobservable ones $\bm{\mu}_u$ (Table~[???]). To collect task-relevant data of these simulated agents, we train a temporary universal policy for the task of interest, $\pi_{temp}(\vc{a}|\vc{s}, \bm{\mu}_o)$, conditioned on the observable model parameters of the agents. The data collected during policy training, which comprises the trajectories of states, actions, and the associated $\bm{\mu_o}$, will be used to train the UDMs. Note that the $\pi_{temp}$ is merely a tool for collecting task-relevant data for training UDM and is discarded afterwards.

% Final products
\noindent\textbf{Learned models.}
We partition the dataset three parts by the range of $\bm{\mu_o}$: a training, a validation, and a testing dataset. For human experiments, we select $???$ out $???$ people as a training set and the other as a testing set. For other control tasks, a training set includes $???$ sets of observable parameters and a testing set has $???$ sets. We then train our 3 LSTM dynamical models : 1) One with training dataset $P(\vc{s}'|\vc{s},\bm{\mu}_o,\vc{a})$, 2) with training and validation datasets $P_{all}(\vc{s}'|\vc{s},\bm{\mu}_o,\vc{a})$ and 3) with testing dataset $P_{test}(\vc{s}'|\vc{s},\bm{\mu}_o,\vc{a})$. 
\sehoon{I don't see Ptest in anywhere in the paper.}
\end{comment}

==> method.tex <==
\section{Method}
%Random notes:
%- Previous work adds noise to some model parameters and train a robust policy or an adaptive policy conditioned on these parameters.

%- The model parameters are either all known to the policy or all unknown to the policy. The former is more convenient to transfer but the policy performance will be reduced. The latter requires fine tuning or another procedure to infer the parameters.

%- In reality, some model parameters will be known while others will be unknown. Our method takes the advantage of known model parameters and predicts the effect of unknown parameters to train a policy for sim-to-real transfer.

%- We propose a new training paradigm that engineers a "Reality Gap" in simulation so that the policy can learn to overcome the gap, in addition to mastering the task. Specifically, we use the real world data to train a "Universal Dynamic Model" conditioned on the observable model parameters. The reality gaps is created by learning separate dynamic models using different observable model parameters for training and testing of the policy.  

%- In addition, we propose a learned representation of the reality gap as an error function conditioned on the state, action and the observable model parameters. The policy will take into account the reality gap predicted by the error function when deciding the optimal action. 

%- Combining the "simulated reality gap" introduced by the universal dynamic models and the learned "error function", our method fully utilizes all the available data from the target environment and measurable model parameters to prepare the policy for sim-to-real transfer.

%- The reality gap we engineer assumes that the reality gap is caused by over-fitting to a small amount of real world data.

%For the dynamic model trained from simulated data, the reality gap we engineer assumes that the real world has the highest entropy in model parameters.


% Introduce the high-level idea: error aware policy
We propose a method to overcome the reality gap in which the parameters affecting the dynamics of the environment and the agent can be divided into observable (easy-to-identify) parameters, such as ??? and ???, and unobservable parameters such as ??? and ???. \sehoon{fill the examples}. \sehoon{Move this sentence to the problem definition section: We denote observable parameters as $\boldsymbol{\mu}_o$ and unobservable parameters as $\boldsymbol{\mu}_u$.}
\karen{I think examples should be presented in the intro and do not need to be repeated here.} \karen{Suggest changing $\mu_u$ to $\nu$ and $\mu_o$ to just $\mu$.}We introduce an \emph{Error-Aware Policy} (EAP), which is explicitly aware of the differences between what is expected in training and what is executed in testing environments, and self-corrects its action accordingly. 
To achieve this goal, we train an additional auxiliary error-prediction function, which takes as inputs an uncorrected action and observable parameters, and outputs the expected state error when a policy trained in one environment is deployed to a different one. 
We train the error-aware policy and the  error prediction function by introducing a novel learning scheme that splits environments with different parameters into training and validation sets.
Our novel approach allows an agent to explicitly identify expected errors and produce corrected actions, which lead to better transfer to environments with unobservable dynamics parameters.
\sehoon{It might be better to have some overview figure.} \karen{Can expand Figure 1 to make it the overview figure. }\karen{Also introduce math symbols as you describe the error function and its input/output.}
% End-of-overview

\sehoon{Move the rest to the proper sections}
To learn the error-prediction function, we introduce a novel approach to training policies with variations in the dynamical parameters \karen{This sentence is logically ambiguous. The novel approach is for training policies with variations or is for training error-prediction function?}. Unlike , domain randomization where the parameters are randomly varied during training \karen{incomplete sentence. grammar!}. 
We sample a set of $n$ different dynamical environments, out of these $n$ environments, we randomly \sehoon{Nominal?} choose one environment as a reference dynamical environment $P_{r}(\mathbf{s'}|\mathbf{s},\mathbf{a},\boldsymbol{\mu}_o)$ as the training set and the rest $n-1$ as a $P_{v_i}(\mathbf{s'}|\mathbf{s},\mathbf{a},\boldsymbol{\mu}_o)$ validation set. Once the policy is trained in $P_{r}$ \karen{Is there a need for subscription r for $P_r$?}, it is then deployed in environments in the validation set to generate data to learn the error-prediction function, while continuing to learn the task in the validation environment \karen{In the intro, you tried to frame it as a meta-learning, but there's no follow up on that in the method section.}. Figure \ref{fig:EAPillustration} illustrates this process of generating data to train the error function by deploying the policy in the validation environments. The function, $E_\phi: (\mathbf{s}, \mathbf{a}, \boldsymbol{\mu}_o) \mapsto \mathbb{R}^n$ is trained simultaneously with EAP to predict the deviation of the future states between the training and testing environments, conditioned on the same current state, the same action, and the same observable model parameters. The output of $E_\phi$ is passed into EAP for computing the optimal action \karen{Why introduced $E_\phi$ so late? You have used the term error-function many times before this. When you finally introduced $E_\phi$, you didn't address it as an error-function, and just called it a function. Why?}.


\subsection{Training Error Prediction Function}
We train an error prediction function $E_{\bm{\phi}} : (\vc{s} ,\vc{a},\bm{\mu_o}) \mapsto \bm{e} \in \mathbb{R}^n$ 
using $P_{r}(\vc{s}'|\vc{s},\bm{\mu}_o,\vc{a})$ and $P_{v_i}(\vc{s}'|\vc{s},\bm{\mu}_o,\vc{a})$. The output error $\bm{e}$ is defined as the deviation of the future state, $(\vc{s}' - \vc{s}_{v_i}') \in \mathbb{R}^n$, generated by two dynamic models $P_r(\vc{s}'|\vc{s}, \vc{a}, \bm{\mu}_o)$ and $P_{v_i}(\vc{s}'|\vc{s},\vc{a}, \bm{\mu}_o)$, for the given state $\vc{s}$, action $\vc{a}$ and observable parameters $\bm{\mu}_o$. Since the differences between the two dynamical environment reflects the reality gap due to the unobservable parameters $\bm{\mu}_u$ and $P_r(\vc{s}'|\vc{s}, \vc{a}, \bm{\mu}_o)$ \karen{Why $P_r$ but not $P_v$?}, our hypothesis is that the error prediction function $R_\phi$ will learn the useful information about the reality gap and inform the EAP to make more effective decisions \karen{It is not clear to me why the error function can capture the information about the unobserved $\mu$? We need some explicit reasoning why error function can be useful. I think there is no way we can reconstruct $\mu_u$ and it is also not the goal of this work. The best we can do is to pool all the information we can observe and from the experiences to learn a predictive model $E_\phi$ and a policy that utilizes it.}. We train our error prediction function $E_\phi(\vc{s}, \vc{a},\mu_o)$ to learn this ``emulated'' domain gap by minimizing the following loss:
\begin{equation} \label{eq:error_prediction_loss}
    L(\bm{\phi}) = \sum_{(\vc{s}^{0},\vc{a}^{0},\bm{\mu}_o,\vc{s}^{T},  \vc{s}_{all}^{T}) \in D} ||E_\phi(\vc{s}^{0}, \vc{a}^{0},\bm{\mu_o})  - (\vc{s}^{T} - \vc{s}_{all}^{T})||^2,
\end{equation}
where $\vc{s}^{T}$ and $\vc{s}_{v_i}^{T}$ are the future state after $T$ steps, $P(\vc{s}'|\vc{s},\bm{\mu}_o,\vc{a})$ and $P_{v_i}(\vc{s}'|\vc{s},\bm{\mu}_o,\vc{a})$, respectively \karen{Update the equation.}. The detailed training procedure is described in Algorithm~\ref{alg:2}. 

% where $\vc{s}' \sim P(\vc{s}'|\vc{s},\bm{\mu}_o,\vc{a})$ and $\vc{s}'_{all} \sim P_{all}(\vc{s}'|\vc{s},\bm{\mu}_o,\vc{a})$.

% \karen{Above equation doesn't make sense. It subtracts two probability distributions and compare that to a vector?}\visak{Hmm, I dont recall writing this, this is actually just a simple regression I will change it}

% To capture the reality-gap we define an error function $\phi : (\bm{s,a,\mu_o}) ->\bm{e}$ that predicts the expected future state error $\bm{e} \in R^n$ (where n is the dimension of the state) when the policy is deployed in different environment. The state error is defined as $(s_{1}^{'} - s_{2}^{1}) \in R^n$ : the state difference generated by two transition functions $P_{1}(s'|s,a)$ and $P_{2}(s'|s,a)$, when action $a$ is taken at state $s$.
% A control policy $\pi : (\bm{s,\mu_o,e}) -> a$, takes the output of the error function as an input and outputs an action that aims to overcome the differences in the dynamics. This policy is trained by formulating it as a model-free reinforcement learning problem. 

\begin{algorithm}[]
\caption{Train an Error Aware Policy.}
\label{alg:1}
\begin{algorithmic}[1]
% \STATE \textbf{Input:} Data-set of $(s,a)$ pairs for n environments : $D_{1..n}$
% \STATE \textbf{Input:} Hold out m (randomly chosen) data as test set : $D_{1..m}$
\STATE \textbf{Input:} Observable parameters for task $\mu_{o}$
\STATE \textbf{Input:} Reference dynamical environment with $\mu_{r}$

\STATE Pre-train $\pi$ for $P(s'|s,a,\mu_{r})$ reference environment with $\vc{e}=0$
\WHILE {not done}
\STATE Sample an environment with $\bm{\mu}_{o}$ from $D_{val}$
\FOR{ each policy update iteration}
\STATE Initialize buffer $B=\{\}$
\STATE Update an error function $\phi$ using Algorithm~\ref{alg:2}
\STATE $B$ = Generate rollouts using Algorithm~\ref{alg:3}
\STATE Update policy $\pi$ using $B_{pol}$ using PPO.
%\ENDFOR

\ENDFOR \label{line:trainingSetEnd}
\ENDWHILE
\RETURN{ $\pi(a|s,\mu_o,e)$}
\end{algorithmic}
\end{algorithm}


\begin{algorithm}
\caption{Train an Error Prediction Function.}
\label{alg:2}
\begin{algorithmic}[1]
\STATE \textbf{Input:} $\mu_o \sim D_{val}$
\STATE \textbf{Input:} Policy $\pi(\vc{a}|\vc{s},\bm{\mu}_{o}, \vc{e})$
\STATE Initialize a buffer $D = \{\}$ 
% \FOR{$i = 1:K$}
\WHILE{not converged}
\STATE Initialize state $\vc{s}^0$ and $\vc{s}_{r}^0, $ 
% \STATE $\vc{s}$ = a state after running a policy $\pi(\vc{a}_{t}|\vc{s}_t,\bm{\mu}_{o}, \vc{e}=0)$ on $P$ for T steps.
\FOR{$t = 0:T$}
\STATE $\vc{a}^t \sim \pi(\vc{a}^{t}|\vc{s}^t,\bm{\mu}_{o}, \vc{e}=0)$ 
\STATE $\vc{s}^{t+1} \sim P(\vc{s}^{t+1}|\vc{s}^t,\vc{a}^t,\bm{\mu}_{o})$
\STATE $\vc{a}_{r}^t \sim \pi(\vc{a}_{r}^{t}|\vc{s}_{r}^t,\bm{\mu}_{o}, \vc{e}=0)$
\STATE $\vc{s}_{r}^{t+1} \sim P(\vc{s}_{r}^{t+1}|\vc{s}_{r}^t,\vc{a}_{r}^t,\bm{\mu}_{o})$  
% \STATE $\vc{s}'_{r,t+1} \sim P_{r}(\vc{s}'|\vc{s},\vc{a},\bm{\mu}_{o})$  
\ENDFOR
\STATE $\vc{e}=\vc{s}^{T}-\vc{s}_{r}^{T}$
\STATE $D = D \cup \{(\vc{s}^0,\vc{a}^0,\bm{\mu}_{o},\vc{s}^{T},\vc{s}_{r}^{T}$)\}
% \STATE Store tuple $(s,a,\mu_{o},\vec{e})$ in buffer $\mathcal{B}$
\ENDWHILE
% \ENDFOR
\STATE minimize the $L(\phi)$ in Eq.~\ref{eq:error_prediction_loss} using $D$.
% \STATE Train neural network $\phi$, with inputs $(s,a,\mu_{o})$ and output $\vec{e}$ using supervised learning with loss $L(\phi)=||f(\phi)-e||^{2}$ 

\RETURN $\phi$
\end{algorithmic}

\end{algorithm}




% % Architecture/definition.
% In our approach the dynamical model is learned from data, a LSTM neural network $P_{\theta}(s'|s,a,\mu_o)$ is used to approximate the dynamics where $\theta$ is the parameters of the LSTM model. In addition to current state $s$ and action $a$ the model also takes as input the observable parameters $\mu_o$ to account for the factors of variation. This learned model is called a "Universal Dynamical Model".


% \subsubsection{Data collection}
% % Data collection in Dart
% For each task, we manually decide certain factors of variations influencing the dynamics such as mass, center of mass location, joint damping, friction, etc. These are described in table 1. We also set a uniform prior for all the quantities, each of which has a set range of values. We then train a robust policy using PPO using DART simulator, uniformly sampling the parameter values at the beginning of each rollout. During training we store the dataset $D_{\mu_{o}} = \{(s_{0},a_{0},\mu_{o})..(s_{t},a_{t},\mu_{o})\}$, which comprises of the state action pairs and observable parameters $\bm{\mu_o}$ for each environment. 

% % Data collection for humans
% For 3D human-like walking we use data from a public dataset of over-ground human walking reported in \cite{dataset2018}. The dataset includes steady state walking data for $40$ different healthy adults with ages ranging from $21$ - $87$.  

% % Data definition/training
% Once our dataset is collected, $D_{\mu_{o}} = \{(s_{0},a_{0},\mu_{o})..(s_{t},a_{t},\mu_{o})\}$,  we train a LSTM neural network to approximate the dynamical model with parameters $\theta$. The model has a history of length ten $L=10$ and we use maximum likelihood optimization described in equation \ref{eq:neg-log} using a negative-log likelihood optimization.


% \begin{equation}
%     \theta^* = \argmax_{\bm{\theta}} \sum_{i = 1}^{n} \sum_{(\bm{s}_{t},\bm{a}_{t},\bm{s}_{t+1}) \in D_{\mu_{o_i}}} \log p_{\theta}(\bm{s_{t+1}}|\bm{s_t},\bm{a_t},\bm{\mu_{o_i}})
%     \label{eq:neg-log}
% \end{equation}

% % Final products
% We split our state-action pairs into three dataset based on $\bm{\mu_o}$ : a training, validation and a testing dataset. Then, we train our 3 LSTM dynamical models : 1)One with training dataset $P(s'|s,\mu_o,a)$, 2) with training and validation data $P_{all}(s'|s,\mu_o,a)$ and 3) with testing data $P_{test}(s'|s,\mu_o,a)$. 

\subsection{Error Aware Policies (EAP)}
\begin{figure}
\centering
\setlength{\tabcolsep}{1pt}
\renewcommand{\arraystretch}{0.7}
  \includegraphics[width=0.37\textwidth,height=4.5cm]{images/Error_function.PNG}
\caption{\small{Definition of a state error generated when a policy trained in one environment is deployed to another test environment. The error function aims to capture this state error for multiple environments.}}
\label{fig:StateError}
\end{figure}

% \begin{figure}
% \centering
% \setlength{\tabcolsep}{1pt}
% \renewcommand{\arraystretch}{0.7}
%   \includegraphics[width=0.5\textwidth,height=4cm]{images/Error.PNG}
% \caption{\karen{Don't need this figure.}}
% \label{fig:ErrorDef}
% \end{figure}



% \textcolor{blue}{Karen notes :Define error function to characterize reality gap
% Define MDP and policy
% Sketch out how we plan to train e and policy simultaneously (Figure 1 and 2)
% Introduce Algorithm 1-3}

% \textcolor{red}{Visak's text below}

We simultaneously train the error prediction function $E_\phi$ and the error aware policy $\pi(\vc{a}|\vc{s},\bm{\mu}_o, \vc{e})$, conditioned on the predicted errors $\vc{e}$, along with the state and the observable parameters (Algorithm \ref{alg:1}). We first pre-train the policy on the reference dynamical environment $P_r$ to maximize the cumulative task reward in the absence of errors (i.e. \vc{e} = \vc{0}). The main training loop iterates between training $E_\phi$ and $\pi$ in the environment $P_{v_i}$ where $i \sim D_{val}$ uniformly sampled from the validation set $D_{val}$. The process of generating data for training error function is described in algorithm \ref{alg:2}. We use a policy gradient method to train EAP (\cite{schulman2017proximal}) which requires the current policy to generate rollouts at each iteration. At each time step of rollout generation, we first query the policy with zero error, $\pi(\vc{a}|\vc{s},\bm{\mu}_o,\vc{e}=0)$, to obtain an action $\tilde{\vc{a}}$, which is subsequently used to query the error prediction function $E_\phi(\vc{s},\tilde{\vc{a}}, \bm{\mu}_o)$, to obtain a predicted error $\tilde{\vc{e}}$. Lastly, we query the final action with $\tilde{\vc{e}}$, $\pi(\vc{a}|\vc{s},\bm{\mu}_o,\tilde{\vc{e}}))$, and executed it in $P_{v_i}$ for rollout generation (Algorithm \ref{alg:3}). 

During testing, an environment is sampled from testing set (previously not seen during training) and the error function is queried without further fine-tuning on new data generated in the environment.


\begin{figure}
\centering
\setlength{\tabcolsep}{1pt}
\renewcommand{\arraystretch}{0.7}
  \includegraphics[width=0.30\textwidth,height=4.2cm]{images2/TrainingMethodology.png}
\caption{\small{Illustration of the method to collect experience tuples to train the error preduction function. Once the policy $\pi(a|s,\mu_o,e=0)$ is trained in the $\mu_r$, the policy is deployed in validation environments $\mu_{v_i}$ to observe the state errors.}\karen{Is this is just a sketch? This figure is not very informative.}}
\label{fig:EAPillustration}
\end{figure}

\subsection{Training details}
% simulator, open ai gym
We use PyDart \cite{pydart} physics simulator to run our experiments combined with Open AI baselines implementation of proximal policy optimization (PPO) \cite{schulman2017proximal}. We use open source bio-mechanics dataset \cite{dataset2018} to obtain the joint angles, velocities and the Center of Mass (CoM) position information for the human agents.  


\begin{algorithm}
\caption{Generate Rollouts}
\label{alg:3}
\begin{algorithmic}[1]
\STATE \textbf{Input:} Observable dynamics parameters $\bm{\mu}_0$.
\STATE \textbf{Input:} Reference dynamical model $P_{r}$
\STATE \textbf{Input:} Current policy $\pi$ and error function $E_(\phi)$
\STATE \textbf{Input:} Replay buffer $B$
\STATE Sample state $\vc{s}$ from initial state distribution $\rho_{0}$ 
\WHILE{not done}
\STATE $\vc{a} \sim \pi(\vc{a}|\vc{s},\bm{\mu}_{o},\vc{e}=0)$ \tcp{original action}
\STATE $\vc{e} = E_\phi(\vc{s}, \vc{a}, \bm{\mu}_{o})$
\STATE $\bar{\vc{a}} \sim \pi(\vc{a}|\vc{s},\bm{\mu}_{o},\vc{e})$ \tcp{error-aware action}
\STATE $\vc{s}'= P_{r}(\vc{s}'|\vc{s},\vc{a},\bm{\mu}_{o})$
\STATE $r = r_{task}(\vc{s},\bar{\vc{a}})$
\STATE $B = B \cup \{(\vc{s},\bar{\vc{a}},r,\vc{s}')\}$
% \STATE Predict error $\vec{e}=f(\phi)$ with inputs $s,a,\mu_{o}$ 
% \STATE Predict action to be taken with $\pi(a|s,\mu_{o},e)$
% \STATE Take one simulation step with  $s'=P_{all}(s'|s,a,\mu_{o})$
% \STATE Compute reward with $r_{task}(s,a)$
% \STATE Store tuple $(s,a,r,s')$ in buffer $B_{pol}$
\STATE $\vc{s}=\vc{s}'$
 
\ENDWHILE
\RETURN $B$
\end{algorithmic}

\end{algorithm}










==> results.tex <==
\section{Results}


\begin{itemize}
    \item Results on learning the dynamics
    \item Results on the open ai gym experiments
    \item Results on the human walking experiments
    \item camparison to baselines
\end{itemize}
